DeepSTL -- From English Requirements to Signal Temporal Logic

Formal methods provide very powerful tools and techniques for the design and analysis of complex systems. Their practical application remains however limited, due to the widely accepted belief that formal methods require extensive expertise and a steep learning curve. Writing correct formal specifications in form of logical formulas is still considered to be a difficult and error prone task. In this paper we propose DeepSTL, a tool and technique for the translation of informal requirements, given as free English sentences, into Signal Temporal Logic (STL), a formal specification language for cyber-physical systems, used both by academia and advanced research labs in industry. A major challenge to devise such a translator is the lack of publicly available informal requirements and formal specifications. We propose a two-step workflow to address this challenge. We first design a grammar-based generation technique of synthetic data, where each output is a random STL formula and its associated set of possible English translations. In the second step, we use a state-of-the-art transformer-based neural translation technique, to train an accurate attentional translator of English to STL. The experimental results show high translation quality for patterns of English requirements that have been well trained, making this workflow promising to be extended for processing more complex translation tasks.

==> review.tex <==
Review #1240A
===========================================================================

Overall merit
-------------
3. Weak accept

Paper summary
-------------
The authors investigate the mapping of requirements expressed in English language and those expressed in STL. The authors analyze which constructs and operators from STL are used with which frequency. The information gained by this analysis is used to construct a grammar which produces requirements in STL such that the operators are used with similar frequencies. The generated requirements and their equivalent in English language are used to train a tool which the authors created. This tool uses machine learning as the authors apply NLP ideas to enable a translation of requirements from English to STL without the use of patterns. The authors investigate with the produced requirement how well their tool works. They also use examples from their analysis of real-world requirements to test their tool.

Strengths
---------
+ Well-motivated, relevant problem
+ Intuitive idea and good presentation of the details of the approach

Weaknesses
----------
- The maturity of the paper can be improved (see detailed comments, and I may have missed alot of similar mistakes).

Comments for authors
--------------------
**Soundness and Novelty:** The paper is positioned to improve translation from unstructured English requirements. The use of NLP for this problem is somewhat novel. It is, however, only tested on requirements which are generated or "clear", i.e., have a straight-forward translation into STL. It would have been interesting to see how the approach works on English requirements of the other defined language qualities, as these should be the tool's goal. I acknowledge that the study is merely a first step towards this goal, but never is this made clear by the authors.


**Significance:** The idea is actually very good. But the significance is not really explained anywhere in the paper clearly. Only in the conclusion (sec7) is it described somewhat, but very sparsely.


**Verifiability and Transparency:** The authors describe very detailed the parameters with which their tool operates. The data and python implementation of the tool are made available for reviewing. The figures are too small to read them, which makes most of the authors' results not verifiable. In particular, the authors claim that they addressed the problem of the lack of publicly available natural language requirements. However, the paper lacks an investigation into threats to validity. 

**Presentation:** Poor. Paper is not mature, see comments below.  Figures are not readable!

**Comments: **

The introduction is quite unusual, the style was not used throughout the paper or in the conclusion Explanations in 4.1 are quite excessive. Maybe a large figure would have been better. 

5.1.3: very detailed/technical. Using an example to demonstrate the technique may be beneficial.

Fig 5 way too small. Figs 3 and 4 are small, too, but acceptable p. 9, ln. 1018: "Which depend on many factors" Why was this not investigated more thoroughly? I.e., investigate how changing one variable affects the results? 

The BLEU score may not be suitable to evaluate the presented tool as the number of words is very low (as stated by the authors)

p. 7, ln. 726: "it is still consistent with the empirical results" how so. How do you define the consistency? Why is there not a similar Fig to Fig 6 in sec4? I.e., why is Fig. 1 a different kind of graph?



**Typos/small remarks:**

p. 1, ln. 67: as well [as]

p. 1, ln. 68: one citation for two arguments / examples? 

p. 1, ln. 108: is this the citation where STL was introduced FIRST?

p. 2, ln. 160: citations for academia and industry separate, please

p. 3, ln. 283: "of an immediate response (IR) specification [if] -> [is] the one from.."

p. 4, ln. 366: This -> These

p. 6, ln. 581: Reachablity -> Reachability

p. 7, ln. 788: How does this compare to the number of different words in the empirical results, section 4?

p. 8, ln. 885: so separated not only by white space but also by comma?

p. 8, ln. 894: "reaches to a upper limit" -> "reaches an upper limit"

p. 8, ln. 898: "Inspired by above BPE execution" what do you mean? The example?  Please state above the example that it is an example of BPE, then

p. 8, ln. 899: "into into"

p. 8, ln. 902: switching time tense

p. 9 Fig7, 8 impossible to read. What do they show? No explanation; explanation in text is insufficient

p. 9, ln. 1029: capitalization

p. 9, ln. 1030: capitalization

Questions for authors to respond to
-----------------------------------
$G$(rise(no question) →$F[0,\infty]$ (no_rebutal_needed))



% ------------------------
% answers to reviewer 1
% ------------------------
% All reviewers:
% We thank all the reviewers for their valuable feedback. Below we provide a detailed answer to their questions.

% Reviewer 1: 
% Significance.
% Our work is motivated by industrial needs. For each product they develop, companies have in general hundreds of pages of requirements specifications written in natural language, and whose fulfilment has to be checked. Our work is a first step to automate this process. From STL there are already tools available to generate automatically generate run-time monitors.

% Presentation:
% Thank you very much for all your suggestions. In the final version we will correct all typos, increase the size of the figures, cut down redundant parts of the text, and use all the way our STL example. In response to your question, F Raise Accept -> G Appreciated






* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #1240B
===========================================================================

Overall merit
-------------
3. Weak accept

Paper summary
-------------
The paper considers the problem of translating CPS natural language requirements to STL.  

To address the lack of publicly available natural language requirements, the authors present a procedure for automatically generating English sentences from STL formulas. They used a transformer-based NLP architecture to efficiently train a reasonably accurate translator from English to STL. 

The authors report on experiments with good results.

Strengths
---------
+ Novelty: first approach of unrestricted learning of NL to TL 
+ translation Important in practice and challenging and interesting 
+ research problem Reasonable results Good presentation Supplementary 
+ material allows inspection and reproduction

Comments for authors
--------------------
[significance and novelty]

The work addresses an instance of the well-known problem of translating NL requirements into formal specifications. The problem is important and very challenging.  

To the best of my knowledge, this is the first work to apply transformers and their attention mechanism to the problem. Related work is discussed as expected. 

I consider the work to have potential impact on the field. 

[soundness]

The work seems to be generally sound. The partition of the work into the two challenges listed in the intro makes sense. Then the five research questions seem to be adequate and they are reasonably addressed in the paper.

I find the research design decisions made by the authors to be reasonable and well justified, given the challenges and limitations in terms of data availability. 

For usefulness in requirements engineering, future work should perhaps consider adding some kind of a confidence measure to each translation, so as to possibly warn users when the machine is not confident in the translation result. 

[presentation]

Very good presentation quality. The style in the beginning of the introduction is a bit unusual, which is refreshing.

If the paper is accepted, perhaps the authors could use the additional space for (1) more examples from the results as in the end of section 6 (2) throughout the paper, some more background, in context, of machine learning terminology (e.g., loss). 

Why is Fig. 6 using a spider / radar diagram and not just a simple bar chart like Fig. 2?

+ 283 "is the one"
+ 1030 "we insert"

[verifiability]

The authors describe the experiments and different steps in preparing the data in reasonable detail.

The collection of data and making it available are a contribution by itself.

The data that the authors collected as well as the code for the experiments are made available in supporting material that seems to be comprehensive and reasonably documented.

Reviewr 2:

Questions for authors to respond to
-----------------------------------
1. It seems that the part that is more difficult for engineers to do when translating informal NL requirements into STL is the formalization of the temporal relations, not the identification of identifiers and numbers. Wouldn't it make more sense to suggest a two step process whereby identifiers and numbers are identified manually or automatically, and when confirmed by an engineer, the complete STL formula is created?  

2. From the text at the end of 6.1 I was unable to understand whether in your current approach identifiers are manually or automatically identified.

% They are automatically identified. A scanner breaks the string of characters in individual words. Numbers, correspond to a particular regular expression. Identifiers, are words that do not belong to a database of commonly used English words.

3. Typically, individual NL requirements are not presented out of context but as part of a large set of requirements for the same system. In this common case, many individual requirements in the set share identifiers. Can you take advantage of that?


4. Please comment on the suggestion to add a confidence measure.



% ------------------------
% Response to reviewer 2
% ------------------------
% We agree with the reviewer. This is an excellent idea. In fact, we considered that user interaction might be necessary, to make sure that the STL translation (parsed again in English), is what the user intended. 

% Answer to question 1:
% Our work assumes no user interaction, so we refer to standard procedure for applications of machine translation in NLP. But we think your advice can be naturally integrated into our method. 

% For recognition of identifiers, in our procedure: 
% (1) A scanner will read the whole sentence, and keep all the words except numbers and special symbols in a word set.
% (2) For every element in the above set, we look up a dictionary that includes all English words in our dataset, and check whether it belongs to this dictionary. If no, we treat it as an identifier, and put it into an identifier list. 
% (3) For every element in the identifier list, we insert a white-blank into each of its character, and replace the original one with the modified version in the input sentence.
% The same is done for numbers, regular expression can be used to recognizing and separating them into digits.

% We think your advice can be directly integrated into Step (2). If we have prior knowledge of what are identifiers, we could directly put them into the identifier list without looking up a dictionary.


% Answer to question 2:
% Since we assume no user interaction in our paper, although the whole procedure above executes automatically, the action of looking up a dictionary is still not a perfect solution. If an identifier happens to be a common English word, e.g., voltage, then we cannot recognize it. That's why we said our method is somewhat 'manually'. An advanced approach is to use Name Entity Recognition (NER) approach in NLP to do the recognition task, and we will leave it for future work.


% Answer to question 3:
% This is a very interesting future direction to go although this proposal is not implemented yet. If we know the shared identifiers, we could definitely take advantage of it by adding several codes in step (2) to match these known identifiers.


% Answer to question 4:
% For the lack of time, we do not put it and we apologize for that. We have computed it, and we will definitely put it in the final version.




* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *
Review #1240C
===========================================================================

Overall merit
-------------
3. Weak accept

Paper summary
-------------
The authors propose to use sequence-to-sequence modeling to translate NL timing requirements into signal temporal logic (STL). The authors first create a NL specification generator by analyzing 130 specifications and associated NL descriptions found in scientific papers and industrial documents. The analysis yielded specification templates and the distribution of temporal operators used in such specifications, which is a rather significant contribution. The generator samples from a three-layer hierarchical syntactic/semantic space of templated NL requirements, which is evaluated based on the templates defined by the domain analysis. Overall, the generator supports 89/130 (68.5%) specifications observed in the domain analysis. The final result is a transformer-based generator with .98-.99 accuracy in translation.

Strengths
---------
+ domain analysis of published STL / NL requirements to establish 
+ grounded theory accounts for NL ambiguity in language translation by 
+ experts reports distribution of generated NL-STL to STL operator space 
+ for clarity

Weaknesses
----------
- limited expressiveness due to biased sources of 130 seed specifications
- lack of comparison with controlled natural language approaches
- missing threats to validity to collect and report limitations of the work

Comments for authors
--------------------
Soundness: The approach begins with a domain analysis to identify syntactic and semantic primitives used to express NL requirements with STL specifications. This yielded canonical templates to describe the domain, plus edge cases and ambiguous and vague uses of NL, which highlights potential domain-specific limitations. One concern is that the 130 seed specifications occur in publications, where the purpose of reporting those specifications is summarize and illustrate an otherwise more complicated specification space. This is a kind of bias not discussed by the authors in threats to validity.



Significance: The authors argue that writing correct STL expressions requires expertise, which can be difficult, as motivation for their work. With high, but imperfect accuracy, the significance of imperfect STL specifications requires expertise to debug those generated specifications. That said, this work opens this new problem to further analysis. A second, yet unaddressed concern, is the extent to which the same or better results could be obtained from an advanced CNL using the same templates described in Section 4.1.

Novelty: The work is a first attempt to develop an automated translator from NL requirements to STL specifications using neural machine translation.

Verifiability and Transparency: The paper is excellent with regard to a transparent analysis of the domain, recognition of limitations of NL requirements (e.g., ambiguity), and multiple assessments comparing the results to the universe of discourse (e.g., see Figures 1, 2 and 6). Moreover, the authors have shared their data for reproducibility. 

Presentation: Text in figures should be at least 8 pt size (see document guidelines, e.g., Fig 2 is difficult to read).

Detailed Comments:

One concern is that the 130 specifications are not a complete, unbiased representation of the space of specification, and that there is a general bias in scientific and industrial publications toward canonical or simple examples to communicate the value of STL. This could mean that this work is only the tip of the iceberg, so to speak. That said, the work reported is detailed and systematic and I can see how others could extend this work, if new insight to more complex and natural expressions arise.

A second concern, however, is that the generator covers a space of restricted natural language NL, similar to a template-based approach used in a controlled natural language, and that this does not fully account for unrestricted NL. In this regard, I wonder how well a more sophisticated CNL would work to solve the same problem? CNLs are only mentioned in Section 2, related work, and the key difference raised by the authors are (1) CNLs and similar work only looks at LTL; and (2) this work looks at the problem of unconstrained NL. The approach described in 5.1 and 5.1.1 generated restricted NL statements, and the difference between LTL and STL in light of the overall approach appears inconsequential: a CNL for LTL could be adapted to STL, no? The authors appear to believe that unrestricted NL only introduces nesting, but I would argue that unrestricted NL could also introduce ambiguity in matters of to which formula nested clauses attach. The paper needs to more fully explore these differences, unfortunately at the cost of removing other useful content.


% ----------------------
% Answer to Reviewer 3
% ----------------------
% For the first concern, we admitted the 130 specifications are biased although their collection are of potential contribution. However, our initial goal is not to merely fit our translator for these specifications. In fact, our primary motivation stems from the needs of our industrial partners where thousands of requirements are already written in natural language, and the main challenge is how to support the extraction of formal specification that can be used to automatize the testing procedures. These practical needs from industry may cause problems for CNL since it has strict requirements for the input language. That's why we want to adopt deep learning and build our own data generator under the situation where no public data is available.



% % Controlled natural language is a valid solution if engineers are originally trained to use these languages when they write the specifications. The reality we face with our industrial partners is that there are already thousands of documents written in natural language and the main challenge is how to support the extraction of formal specification that can be used to automatize the testing procedures. Our work provides the engineers a starting point, and as the reviewer says this is "only the tip of the iceberg". 


% For the second concern, although the preliminary version of the data generator in section 5 is not perfect, we think it would be one of our primary contributions based on:

% (1) Anyone or companies interested could conveniently change the supported grammar in our generator with corresponding English translations to make it cover more scenarios.
% (2) Given that NL at present is manually provided for the generator, we admit this will unavoidably lead to restricted language. But with our efforts, although not shown in the paper due to space, it is not difficult for us to generate more than 100,000 fluent synonymous translations for a complex STL formula, the number of which may be beyond the capability that a CNL-translator can handle. Besides, if data augmentation techniques in NLP are adopted - suppose n variants can be automatically generated from one translation, then we could finally get overall n^100000 translations, many of which may embody various language features like ambiguity and vagueness. 
% (3) With the mention of data augmentation in the last point, this work will potentially attract researchers in other community, especially from NLP, and boost more interesting research directions. Since CNL-based translation has accumulated much experience in this field especially in extracting syntactical and semantic information, we believe it is very promising to integrate these two approaches together for our shared research problem.

==> review_response.tex <==
We thank all the reviewers for their valuable feedback. 

Before providing detailed answers, we would like to restate our research significance - This is the first work, guided by empirical study, to adopt deep learning to address the problem of automatic translation from English requirements to STL. The corpus generator and the corresponding data-set fill in the blank of scarcity of training data in this field, and would have an important impact on follow-up research.

------------------------
Answers to reviewer 1
------------------------
Many thanks for all your suggestions. We apologize for not providing the highest presentation quality due to limited time. In the final version, we promise to: (1) provide more examples in section 5.1.3 and 6.3.3; (2) change style of Fig.6; (3) illustrate effects of different hyper-parameters in training; (4) emphasize significance and polish other presentations.


------------------------
Answers to reviewer 2
------------------------
We agree with the reviewer's excellent idea. 

Answer to question 1:
Our work assumes no user interaction, so we refer to standard procedure of automatic machine translation from NLP. 

For recognition of identifiers during testing, in our procedure: 
(1) A scanner will read the whole sentence, putting all the words except numbers and special symbols in one Python set.
(2) For every element in the above set, we check whether it belongs to a dictionary that includes all English words in our data-set. If no, we treat it as an identifier, and put it into an identifier list. 
(3) For every element in the identifier list, it is split into characters separated by white-spaces (e.g., PWM -> P W M), and the original identifier in the input sentence will be replaced by its modified version.
The same splitting operation is done for numbers, and regular expression can be used for recognition.

We think your advice can be directly integrated into Step (2). If we have prior knowledge of what are identifiers, it would be beneficial to directly put them into the identifier list without looking up a dictionary.


Answer to question 2:
Although our identifier recognition procedure executes automatically, the action of looking up a dictionary is still not a perfect solution. If an identifier happens to be a common English word, e.g., voltage, we cannot automatically recognize it. That's why we say our method is somewhat 'manually'. An advanced approach is to use Name Entity Recognition (NER) approach from NLP, which will be explored in the future.


Answer to question 3:
This is a very interesting future direction despite of no implementation currently. If we know the shared identifiers, we could definitely take advantage of it by modifying step (2) to match these known identifiers.


Answer to question 4:
For limited time, we did not put confidence and we apologize for that. We have computed it, and we will definitely add it in the final version.

----------------------
Answer to reviewer 3
----------------------
For the first concern, we admit the 130 specifications are biased. However, our goal is not to merely fit our translator for these specifications. In fact, our primary motivation stems from the needs of our industrial partners where thousands of requirements are already written in natural language, and the main challenge is how to support the extraction of formal specifications that can be used to automatize the testing procedures. These practical needs from industry may cause problems for the CNL approach since it sets strict rules for the input language. That's why we resort to deep learning.

Besides, the design of our generator makes it convenient to change the supported grammar with reused English translations so that more scenarios can be covered - not restricted to the 130 specifications.

For the second concern, 
Despite that the NL in our generator is produced through a rule-based method with human intervention, we can still generate enormous fluent synonymous translations for relatively complex STL formulas. Besides, the significance of the generator does not stop from here - if standard data augmentation techniques from NLP are adopted, theoretically we are confident to provide much more utterances in exponential order based on what we have generated. These new variants may involve diverse language features like ambiguity and vagueness. We do not implement this mainly because the goal of Section 6 is to test the performance of three mainstream machine translation architectures. As a starting point, it is better controlled to train them in a closed environment. In the future, we are very interested to compare CNL approach and learn something from it to make the overall solutions more effective.



----------------------------------------------
We thank all reviewers for their constructive feedback. Below we provide a detailed answer to their questions. As pointed out, this work is just the beginning of a long journey, and we plan to use the valuable suggestions for improving the final version, and also as an inspiration for future research.

1. Reviewer 1

(1) Only tested on clear requirements: We agree, and we plan in the future to expand the work as suggested. We will improve the final version by better pointing out the current limitations.

(2) Significance. We will clarify in the final version. The paper was motivated by industrial needs. For each product, companies have in general hundreds of pages of NL requirement-specifications, whose fulfilment has to be checked. Our work is a first step to automate this process. From STL specifications, there are already tools available, that automatically generate run-time monitors. 

(3) Presentation: Thank you very much for all your suggestions. In the final version we will correct all typos, increase the size of the figures, draw them in the same style, remove redundant parts of the text, and use all the way our STL example. In the final version we will discuss limitations and threats to validity.

In response to your question: 
$F[author-response, acceptance-notification]$ (rise(Accept)) -> $G$(Appreciated)

2. Reviewer 2

(1) Identifiers and numbers: This is an excellent idea that we will certainly investigate in the future. In fact, user interaction is necessary anyway, to remove ambiguities in the translation.

(2) Identifiers: They are automatically identified, by checking that they do not belong to our dataset of commonly used English words, or the English formulation of STL operators. This is not yet perfect though, as a user may decide to use words in this dataset as identifiers, too.

(3) Context: Yes. In fact, many industrial specifications, contain tables at the beginning, introducing the identifiers, their type, their range, etc. In the future, we plan to extend our tool to consider such tables.

(4) Confidence measure: This is an excellent idea and we will add it to the final version of the paper. As the translation of each word is given by a SoftMax function, we can compute the overall confidence measure of the sentence, as a joint probability.

3. Reviewer 3

(1) Incompleteness and bias: The 130 specifications considered are indeed just the tip of the iceberg. The results of this paper can be improved in future work by adding training examples drawn for example from other distributions (a good candidate is the uniform distribution), or from timing diagrams (these are widely used in the analog- and digital-circuits community). We will add a discussion on this topic.

(2) Generator coverage: Extending an LTL-CNL to an STL-CNL is indeed possible, and taking advantage of available specifications in an LTL-CNL for training purposes is an excellent idea. However, LTL, STL, and CNLs in general, have a long history, and they have still not become mainstream. Our NL generator aims to close this gap; but many more examples, taken from industrial documents, or obtained through user interaction with our tool, will be necessary for a truly unconstrained NL. These examples may also highlight desired extensions of STL, too.

We hope this work will raise the interest of other researchers so that more data can be generated.
